Two Counterexamples to Tokenization and the Noiseless Channel

In Tokenization and the Noiseless Channel (Zouhar et al., 2023a), R\'enyi efficiency is suggested as an intrinsic mechanism for evaluating a tokenizer: for NLP tasks, the tokenizer which leads to the highest R\'enyi efficiency of the unigram distribution should be chosen. The R\'enyi efficiency is thus treated as a predictor of downstream performance (e.g., predicting BLEU for a machine translation task), without the expensive step of training multiple models with different tokenizers. Although useful, the predictive power of this metric is not perfect, and the authors note there are additional qualities of a good tokenization scheme that R\'enyi efficiency alone cannot capture. We describe two variants of BPE tokenization which can arbitrarily increase R\'enyi efficiency while decreasing the downstream model performance. These counterexamples expose cases where R\'enyi efficiency fails as an intrinsic tokenization metric and thus give insight for building more accurate predictors.

==> macros.tex <==
%%% Comment macros
\definecolor{TodoColor}{rgb}{1,0.7,0.6}
\newcommand{\todonote}[3][]{\todo[color=#2,size=\scriptsize,fancyline,caption={},#1]{#3}}
\newcommand{\vilem}[2][]{\todonote[#1]{pink}{\textbf{Vilém:} #2}}
\newcommand{\Vilem}[2][]{\vilem[inline,#1,size=\footnotesize]{#2}}
\newcommand{\marco}[2][]{\todonote[#1]{orange!20}{\textbf{Marco:} #2}}
\newcommand{\Marco}[2][]{\marco[inline,#1,size=\footnotesize]{#2}}
\newcommand{\sangwhan}[2][]{\todonote[#1]{green!20}{\textbf{Sangwhan:} #2}}
\newcommand{\Sangwhan}[2][]{\sangwhan[inline,#1,size=\footnotesize]{#2}}
\newcommand{\todox}[2][]{\todonote[#1]{TodoColor}{\textbf{TODO:} #2}}
\newcommand{\TODOX}[2][]{\todox[inline,#1,size=\footnotesize]{#2}}
\newcommand{\TODOMARK}{%
    \raisebox{-1mm}{\todo[
        color=TodoColor,size=\scriptsize,
        fancyline,caption={},
        inline,inlinewidth=10mm,noinlinepar
    ]{TODO}}\xspace%
}
\newcommand{\response}[1]{\vspace{3pt}\hrule\vspace{3pt}\textbf{#1:}}

\newmdenv[
  linecolor=black,
  linewidth=1.2pt,
  topline=false,
  bottomline=false,
  rightline=false,
  innertopmargin=0mm,
  innerbottommargin=-0.5mm,
  innerleftmargin=1mm,
  skipabove=1.1\topsep,
  skipbelow=0.5\topsep,
]{quotebox}


% Misc macros
\newcommand{\hrefEmail}[2]{\texttt{\href{mailto:#1}{\color{black}{\fontsize{11}{9}\selectfont #2}}}}
\newcommand{\proofpreamble}{\fontsize{8.2}{2}\selectfont}
\newenvironment{equationhalf}[1]
{\begin{minipage}{#1\linewidth}
\begin{equation}
}
{
\end{equation}
\end{minipage}
}

% lexical macros
\newcommand{\whitezero}{\textcolor{white}{0}}
\newcommand{\merge}{\mu}
\newcommand{\merges}{\boldsymbol{\merge}}
\newcommand{\mop}[2]{\ensuremath{[#1,#2]}}
\newcommand{\mopt}[2]{\ensuremath{[\texttt{#1},\texttt{#2}]}}
\newcommand{\str}{\boldsymbol{x}}
\newcommand{\vocab}{\ensuremath{\mathcal{V}}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\dec}{\scalebox{0.9}{\textsc{Dec}}}
\newcommand{\sub}{\scalebox{0.9}{\textsc{Sub}}}
\newcommand{\freq}{\scalebox{0.9}{\textsc{Freq}}}
\newcommand{\rankbot}{\ensuremath{r_\bot}}
\newcommand{\ranktop}{\ensuremath{r_\top}}
\newcommand{\ent}{\mathrm{H}}
\newcommand{\eff}{\mathrm{Eff}}
\newcommand{\pdelta}{p_{\scaleto{\vocab}{4pt}}}
\newcommand{\rvDelta}{\mathrm{W}_{\scaleto{\vocab}{4pt}}}
\newcommand{\cv}{c_{\scaleto{\vocab}{4pt}}}
\newcommand{\cvp}{c_{\scaleto{\ensuremath{\mathcal{V}'}}{4pt}}}
\newcommand{\pv}{p_{\scaleto{\vocab}{4pt}}}
\newcommand{\pvp}{p_{\scaleto{\ensuremath{\mathcal{V}'}}{4pt}}}
\newcommand{\Tv}{T_{\scaleto{\vocab}{4pt}}}
\newcommand{\Tvp}{T_{\scaleto{\ensuremath{\mathcal{V}'}}{4pt}}}


\newcommand{\prooftext}[1]{\textit{\textcolor{gray}{#1}}}

% hack for blank footnotes
\let\svthefootnote\thefootnote
\newcommand\blankfootnote[1]{%
  \let\thefootnote\relax\footnotetext{#1}%
  \let\thefootnote\svthefootnote%
}


\definecolor{ethblue}{rgb}{0,0.1,0.4}
\newcommand{\ethletter}{\hspace{-0.5mm}\text{
    \fontfamily{phv}\fontseries{bx}\fontsize{8}{\baselineskip}\selectfont
    \textit{\textbf{\color{ethblue}{E}}}}
}
\newcommand{\tokyoletter}{
    \text{\raisebox{-0.3mm}{\includegraphics[width=3mm]{img/tokyo_tech.png}}}
}

==> tables/all_metrics.tex <==
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.075}
\resizebox{\linewidth}{!}{
\begin{tabular}{
>{\hspace{-1mm}}c<{\hspace{-4mm}}
r
r
c
c
c
}
\toprule

\bf Tokenizer & \hspace{1mm} $\boldsymbol N$ & $\boldsymbol k$ & $\textbf{PCT} \uparrow$ & $\textbf{SEQ} \downarrow$ & \bf BLEU \\
\midrule
\textsc{Base.} (4k/4k)
& - & - & 0.461 & 25.50 & 33.74\\

\hdashline

\multirow{ 4}{*}{\textsc{Random-Drop}}
& 2k & 500 & 0.356 & 31.46 & 33.39\\
& 2k & 1k & 0.233 & 40.37 & 32.76\\
& 4k & 500 & 0.405 & 29.23 & 33.72\\
& 4k & 1k & 0.352 & 33.37 & 33.40\\

\hdashline

\multirow{ 2}{*}{\shortstack[c]{\textsc{Random-Drop} \\ (4.5k/4.5k)}}
& 2k & 500 & 0.356 & 31.46 & 33.35\\
& 4.5k & 500 & 0.402 & 27.93 & 33.69\\


\hdashline

\multirow{ 4}{*}{\textsc{Duplicate}}
& 100 & 3 & 0.590 & 25.50 & 32.37\\
& 100 & 5 & 0.633 & 25.50 & 31.32\\
& 500 & 3 & 0.571 & 25.50 & 32.26\\
& 500 & 5 & 0.605 & 25.50 & N/A\\

\midrule
\textsc{Base.} (6k/6k)
& - & - & 0.405 & 24.05 & 33.94\\

\hdashline

\multirow{ 4}{*}{\textsc{Random-Drop}}
& 2k & 500 & 0.312 & 29.46 & 33.46\\
& 2k & 1k & 0.210 & 37.64 & 32.86\\
& 6k & 500 & 0.383 & 25.79 & 33.69\\
& 6k & 1k & 0.354 & 27.92 & 33.60\\

\hdashline

\multirow{ 2}{*}{\shortstack[c]{\textsc{Random-Drop} \\ (6.5k/6.5k)}}
& 2k & 500 & 0.303 & 29.19 & 33.37\\
& 6.5k & 500 & 0.376 & 25.35 & 33.69\\

\hdashline

\multirow{ 4}{*}{\textsc{Duplicate}} 
& 100 & 3 & 0.525 & 24.05 & 32.27\\
& 100 & 5 & 0.574 & 24.05 & 31.60\\
& 500 & 3 & 0.522 & 24.05 & 32.43\\
& 500 & 5 & 0.562 & 24.05 & 30.57\\

\midrule
\textsc{Base.} (9k/9k)
& - & - & 0.356 & 22.91 & 33.60\\

\hdashline

\multirow{ 4}{*}{\textsc{Random-Drop}}
& 2k & 500 & 0.275 & 28.04 & 33.35\\
& 2k & 1k & 0.190 & 35.56 & 32.73\\
& 9k & 500 & 0.347 & 23.81 & 33.68\\
& 9k & 1k & 0.332 & 25.07 & 33.59\\

\hdashline

\multirow{ 2}{*}{\shortstack[c]{\textsc{Random-Drop} \\ (9.5k/9.5k)}}
& 2k & 500 & 0.273 & 27.70 & 33.31\\
& 9.5k & 500 & 0.339 & 23.83 & 33.60\\

\hdashline

\multirow{ 4}{*}{\textsc{Duplicate}} 
& 100 & 3 & 0.456 & 22.91 & 32.48\\
& 100 & 5 & 0.507 & 22.91 & 31.64\\
& 500 & 3 & 0.469 & 22.91 & 32.42\\
& 500 & 5 & 0.514 & 22.91 & 30.93\\


\midrule
\textsc{Base.} (14k/14k)
& - & - & 0.308 & 21.95 & 33.59\\

\hdashline

\multirow{ 4}{*}{\textsc{Random-Drop}}
& 2k & 500 & 0.244 & 26.61 & 33.05\\
& 2k & 1k & 0.178 & 33.03 & 32.63\\
& 14k & 500 & 0.301 & 22.67 & 33.41\\
& 14k & 1k & 0.295 & 23.33 & 33.35\\

\hdashline

\multirow{ 2}{*}{\shortstack[c]{\textsc{Random-Drop} \\ (14.5k/14.5k)}}
& 2k & 500 & 0.241 & 26.50 & 33.11\\
& 14.5k & 500 & 0.301 & 22.43 & 33.49\\

\hdashline

\multirow{ 4}{*}{\textsc{Duplicate}}
& 100 & 3 & 0.377 & 21.95 & 32.49\\
& 100 & 5 & 0.432 & 21.95 & 31.45\\
& 500 & 3 & 0.411 & 21.95 & 32.55\\
& 500 & 5 & 0.458 & 21.95 & 30.70\\

\bottomrule
\end{tabular}
}
\caption{The Percentile Frequency (\textbf{PCT}) and Sequence Length (\textbf{SEQ}) predictors compared with the BLEU score. \textbf{PCT} positively correlates with BLEU, while \textbf{SEQ} correlates negatively.}
\label{tab:all_metrics}
\end{table}




==> tables/mt_duplication.tex <==
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{0.75\linewidth}{!}{%
\begin{tabular}{
c<{\hspace{-3mm}}
l<{\hspace{-3mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
}
\toprule
\bf Tokenizer & $\boldsymbol N$ & $\boldsymbol k$ & $\boldsymbol{\eff_\alpha}$ & \bf BLEU \\
\midrule
\textsc{Baseline (4k/4k)} & - & - & $0.474$ & $33.74$ \\ \hdashline
\multirow{ 4}{*}{\shortstack[c]{\textsc{Duplication}\\ \textsc{(4k/4k)}}} 
& $100$ & $3$ & $0.594$ & $32.37$  \\
& $100$ & $5$ & $0.648$ & $31.32$ \\
& $500$ & $3$ & $0.583$ & $32.26$ \\
& $500$ & $5$ & $0.627$ & N/A \\
\midrule
\textsc{Baseline (6k/6k)~~~~~} & - & - & $0.444$ & $33.94$ \\ \hdashline
\multirow{ 4}{*}{\shortstack[c]{\textsc{Duplication}\\ \textsc{(6k/6k)}}} 
& $100$ & $3$ & $0.560$ & $32.27$ \\
& $100$ & $5$ & $0.612$ & $31.60$ \\
& $500$ & $3$ & $0.552$ & $32.43$ \\
& $500$ & $5$ & $0.598$ & $30.57$ \\
\midrule
\textsc{Baseline (9k/9k)} & - & - & $0.418$ & $33.60$ \\ \hdashline
\multirow{ 4}{*}{\shortstack[c]{\textsc{Duplication}\\ \textsc{(9k/9k)}}} 
& $100$ & $3$ & $0.530$ & $32.48$  \\
& $100$ & $5$ & $0.581$ & $31.64$ \\
& $500$ & $3$ & $0.525$ & $32.42$ \\
& $500$ & $5$ & $0.572$ & $30.93$ \\
\midrule
\textsc{Baseline (14k/14k)} & - & - & $0.394$ & $33.59$ \\ \hdashline
\multirow{ 4}{*}{\shortstack[c]{\textsc{Duplication}\\ \textsc{(14k/14k)}}} 
& $100$ & $3$ & $0.501$ & $32.49$ \\
& $100$ & $5$ & $0.551$ & $31.45$ \\
& $500$ & $3$ & $0.498$ & $32.55$ \\
& $500$ & $5$ & $0.545$ & $30.70$ \\
\bottomrule
\end{tabular}
}
\caption{Experimental results for the \textsc{Duplication}. For each \textsc{Baseline} tokenizer, we compare to \textsc{Duplication} (based on the respective \textsc{Baseline}) with various hyperparameters. The average over three training runs is used for all experiments.
N/A: This configuration achieved less than 5 BLEU across several trials, so it is omitted.
}
\label{tbl:duplication_results}
\end{table}(base)

==> tables/mt_random_drop.tex <==
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{
>{\hspace{-2mm}}c<{\hspace{-4mm}}
c<{\hspace{-3mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
}
\toprule
&&&\multicolumn{2}{c}{\bf Overall} &\multicolumn{2}{c}{\bf Best} \\
\bf Tokenizer & $\boldsymbol N$ & $\boldsymbol k$ & $\boldsymbol{\eff_\alpha}$ & \bf BLEU &  $\boldsymbol{\eff_\alpha}$* & \bf BLEU* \\
\midrule
\textsc{Baseline (4k/4k)} & - & - & $0.474$ & $33.74$ & - & - \\ \hdashline
\multirow{ 4}{*}{\shortstack[c]{\textsc{Random-Drop}\\ (4k/4k)}} 
& 2k & 500 & $0.500$ & $33.39$ & $0.504$ & $33.48$ \\
& 2k & 1k & $0.474$ & $32.76$ & $0.483$ & $32.89$ \\
& 4k & 500 & $0.497$ & $33.72$ & $0.498$ & $33.85$ \\
& 4k & 1k & $0.506$ & $33.40$ & $0.518$ & $33.48$ \\ \hdashline
\multirow{ 2}{*}{\shortstack[c]{\textsc{Random-Drop}\\ (4.5k/4.5k)}} 
& 2k & 500 & $0.491$ & $33.35$ & $0.495$ & $33.37$ \\
& 4.5k & 500 & $0.485$ & $33.69$ & $0.487$ & $33.81$ \\
\midrule
\textsc{Baseline (6k/6k)} & - & - & $0.444$ & $33.94$ & - & - \\ \hdashline
\multirow{ 4}{*}{\shortstack[c]{\textsc{Random-Drop}\\ (6k/6k)}} 
& 2k & 500 & $0.468$ & $33.46$ & $0.471$ & $33.46$ \\
& 2k & 1k & $0.441$ & $32.86$ & $0.445$ & $33.03$ \\
& 6k & 500 & $0.458$ & $33.69$ & $0.458$ & $33.94$ \\
& 6k & 1k & $0.473$ & $33.60$ & $0.472$ & $33.71$ \\ \hdashline
\multirow{ 2}{*}{\shortstack[c]{\textsc{Random-Drop}\\ (6.5k/6.5k)}} 
& 2k & 500 & $0.462$ & $33.37$ & $0.464$ & $33.44$ \\
& 6.5k & 500 & $0.451$ & $33.69$ & $0.453$ & $33.70$ \\

\midrule
\textsc{Baseline (9k/9k)} & - & - & $0.418$ & $33.60$ & - & - \\ \hdashline
\multirow{ 4}{*}{\shortstack[c]{\textsc{Random-Drop}\\ (9k/9k)}}
& 2k & 500 & $0.441$ & $33.35$ & $0.440$ & $33.45$ \\
& 2k & 1k & $0.426$ & $32.73$ & $0.440$ & $32.87$ \\
& 9k & 500 & $0.426$ & $33.68$ & $0.425$ & $33.74$ \\
& 9k & 1k & $0.435$ & $33.59$ & $0.436$ & $33.66$ \\ \hdashline
\multirow{ 2}{*}{\shortstack[c]{\textsc{Random-Drop}\\ (9.5k/9.5k)}} 
& 2k & 500   & $0.440$ & $33.31$ & $0.440$ & $33.33$ \\
& 9.5k & 500 & $0.423$ & $33.60$ & $0.423$ & $33.71$ \\
\midrule
\textsc{Baseline (14k/14k)} & - & - & $0.394$ & $33.59$ & - & - \\ \hdashline
\multirow{ 4}{*}{\shortstack[c]{\textsc{Random-Drop}\\ (14k/14k)}} 
& 2k & 500  & $0.415$ & $33.05$ & $0.417$ & $33.09$ \\
& 2k & 1k   & $0.409$ & $32.63$ & $0.416$ & $32.84$ \\
& 14k & 500 & $0.399$ & $33.41$ & $0.399$ & $33.54$ \\
& 14k & 1k  & $0.405$ & $33.35$ & $0.404$ & $33.45$ \\ \hdashline
\multirow{ 2}{*}{\shortstack[c]{\textsc{Random-Drop}\\ (14.5k/14.5k)}} 
& 2k    & 500 & $0.412$ & $33.11$ & $0.415$ & $33.17$ \\
& 14.5k & 500 & $0.396$ & $33.49$ & $0.396$ & $33.54$ \\
\bottomrule
\end{tabular}}
\caption{Experimental results for the \textsc{Random-Drop}. For each \textsc{Baseline} tokenizer, we compare to \textsc{Random-Drop} (based on the respective \textsc{Baseline}) with various hyperparameters. \textbf{Overall} and \textbf{Best} are based on three tokenizer seeds.
}
\label{tbl:random_drop_results}
\end{table}






==> tables/verify_duplication.tex <==
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{
\begin{tabular}{
>{\hspace{-1mm}}c<{\hspace{-4mm}}
l<{\hspace{-3mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
c<{\hspace{-4mm}}
c<{\hspace{-4mm}}
c<{\hspace{-2mm}}
}
\toprule
\bf Tokenizer & \hspace{1mm} $\boldsymbol N$ & $\boldsymbol k$ & $\boldsymbol{\ent}$ & $\boldsymbol{\ent_{0.5}}$ & $\boldsymbol{\ent_{3}}$ & $\boldsymbol{\eff}$ & $\boldsymbol{\eff_{0.5}}$ & $\boldsymbol{\eff_{3}}$ \\
\midrule
\multirow{ 4}{*}{\shortstack[c]{\textsc{BPE}\\(8k)}}

& - & - & 10.16 & 11.82 & 6.17 & 1.13 & 1.32 & 0.69\\
& 100 & 3 & 10.86 & 12.01 & 7.75 & 1.21 & 1.33 & 0.86\\
& 100 & 5 & 11.18 & 12.14 & 8.48 & 1.24 & 1.34 & 0.94\\
& 500 & 3 & 11.16 & 12.28 & 7.75 & 1.23 & 1.35 & 0.85\\
& 500 & 5 & 11.62 & 12.56 & 8.49 & 1.26 & 1.36 & 0.92\\

\midrule
\multirow{ 4}{*}{\shortstack[c]{\textsc{BPE}\\(28k)}}

& - & - & 10.65 & 13.29 & 5.83 & 1.04 & 1.30 & 0.57\\
& 100 & 3 & 11.37 & 13.40 & 7.42 & 1.11 & 1.31 & 0.72\\
& 100 & 5 & 11.71 & 13.48 & 8.15 & 1.14 & 1.32 & 0.80\\
& 500 & 3 & 11.59 & 13.54 & 7.42 & 1.13 & 1.32 & 0.72\\
& 500 & 5 & 12.02 & 13.71 & 8.16 & 1.17 & 1.33 & 0.79\\

\midrule
\multirow{ 4}{*}{\shortstack[c]{\textsc{BPE}\\(50k)\\(GPT2)}}

& - & - & 10.76 & 13.66 & 5.93 & 1.00 & 1.27 & 0.55\\
& 100 & 3 & 11.49 & 13.77 & 7.52 & 1.07 & 1.28 & 0.70\\
& 100 & 5 & 11.83 & 13.83 & 8.26 & 1.10 & 1.29 & 0.77\\
& 500 & 3 & 11.70 & 13.89 & 7.52 & 1.09 & 1.29 & 0.70\\
& 500 & 5 & 12.13 & 14.04 & 8.26 & 1.12 & 1.30 & 0.77\\

\bottomrule
\end{tabular}
}
\caption{Entropies and efficiencies of various tokenizers and their \textsc{Duplication} modifications on 1M English Wikipedia sentences. All quantities increase from the first row in each section, which corresponds to the underlying tokenizer.}
\vspace{8mm}
\label{tab:verify_duplication}
\end{table}

==> tables/verify_random_drop.tex <==
\begin{table}[htbp]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{
>{\hspace{-1mm}}c<{\hspace{-4mm}}
l<{\hspace{-3mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
c<{\hspace{-2mm}}
c<{\hspace{-4mm}}
c<{\hspace{-4mm}}
c<{\hspace{-2mm}}
}
\toprule
\bf Tokenizer & $\boldsymbol N$ & $\boldsymbol k$ & $\boldsymbol{\ent}$ & $\boldsymbol{\ent_{0.5}}$ & $\boldsymbol{\ent_{3}}$ & $\boldsymbol{\eff}$ & $\boldsymbol{\eff_{0.5}}$ & $\boldsymbol{\eff_{3}}$ \\
\midrule
\multirow{ 4}{*}{\shortstack[c]{\textsc{BPE}\\(8k)}}

&  &  & 10.16 & 11.82 & 6.17 & 1.13 & 1.32 & 0.69\\
& 2500 & 500 & 8.42 & 11.11 & 5.11 & 0.94 & 1.24 & 0.57\\
& 2500 & 1000 & 7.72 & 10.66 & 5.10 & 0.87 & 1.20 & 0.58\\
& $\infty$ & 500 & 9.51 & 11.49 & 6.20 & 1.06 & 1.29 & 0.69\\
& $\infty$ & 1000 & 8.90 & 11.19 & 5.80 & 1.00 & 1.26 & 0.65\\

\midrule
\multirow{ 4}{*}{\shortstack[c]{\textsc{BPE}\\(28k)}}

&  &  & 10.65 & 13.29 & 5.83 & 1.04 & 1.30 & 0.57\\
& 2500 & 500 & 9.16 & 12.74 & 5.53 & 0.90 & 1.25 & 0.54\\
& 2500 & 1000 & 7.75 & 12.23 & 4.66 & 0.76 & 1.20 & 0.46\\
& $\infty$ & 500 & 10.50 & 13.19 & 5.94 & 1.03 & 1.29 & 0.58\\
& $\infty$ & 1000 & 10.34 & 13.10 & 5.98 & 1.01 & 1.28 & 0.59\\

\midrule
\multirow{ 4}{*}{\shortstack[c]{\textsc{BPE}\\(50k)\\(GPT2)}}

&  &  & 10.76 & 13.66 & 5.93 & 1.00 & 1.27 & 0.55\\
& 2500 & 500 & 9.55 & 13.22 & 5.90 & 0.89 & 1.23 & 0.55\\
& 2500 & 1000 & 8.27 & 12.77 & 5.17 & 0.77 & 1.19 & 0.48\\
& $\infty$ & 500 & 10.70 & 13.61 & 5.99 & 1.00 & 1.27 & 0.56\\
& $\infty$ & 1000 & 10.63 & 13.56 & 6.00 & 0.99 & 1.26 & 0.56\\

\bottomrule
\end{tabular}
}
\caption{Entropies and efficiencies of various tokenizers and their \textsc{Random-Drop} modifications on 1M English Wikipedia sentences. All quantities increase from the first row in each section.}
\label{tab:verify_drop_bpe}
\end{table}
